A quantitative probabilistic relational Hoare logic

We introduce eRHL, a program logic for reasoning about relational expectation properties of pairs of probabilistic programs. eRHL is quantitative, i.e., its pre- and post-conditions take values in the extended non-negative reals. Thanks to its quantitative assertions, eRHL overcomes randomness alignment restrictions from prior logics, including PRHL, a popular relational program logic used to reason about security of cryptographic constructions, and apRHL, a variant of PRHL for differential privacy. As a result, eRHL is the first relational probabilistic program logic to be supported by non-trivial soundness and completeness results for all almost surely terminating programs. We show that eRHL is sound and complete with respect to program equivalence, statistical distance, and differential privacy. We also show that every PRHL judgment is valid iff it is provable in eRHL. We showcase the practical benefits of eRHL with examples that are beyond reach of PRHL and apRHL.

==> cases.tex <==
\section{Case studies} \label{s:cases}
\MA{fix sectioning}
This section showcases the expressiveness of \ERHL. We consider both
examples that are out of scope of previous logics (two samplings
vs. one sampling, rejection sampling, randomized response, privacy
amplification by subsampling) as well as examples that are provable in
previous logics (PRF/PRP switching lemma, algorithmic stability of
Stochastic Gradient Descent).



\subsection{Program equivalence}



\subsection{Total variation}


\subsection{Differential privacy}



\subsection{Kantorovich distance}
\label{sec:sgd}
\newcommand{\loss}{\ell}
\newcommand{\grad}{\nabla}
\newcommand{\diffone}{\simeq_1}
\newcommand{\sgd}{\cmd_{\mathsf{SGD}}}

\emph{Algorithmic stability} expresses the tendency of a learning mechanism to produce models that have similar performance on unseen examples
and on the training dataset~\cite{Bousquet}.
We revisit algorithmic stability of \emph{Stochastic Gradient Descent (SGD)},
a classic testbed for verification of relational expected properties,
modeled as follows:
\[
  \sgd \defsym\pw{
    \var{w} <- \var{w}_0; \var{t} <- 0 ;\\
    \WHILE \var{t} < T
    \DO{
      \var{s} <* \var{S};\\
      \var{g} <- \grad(\loss(\var{s}))(\var{w});\\
      \var{w} <- \var{w} - \var{\alpha_t} \cdot \var{g};\\
      \var{t} <-\var{t}+1
    }
  }
\]
This program runs on a
set of examples $S\in A^n$ and ``learns'' a sequence of parameters
$w\in \Real^d$, repeatedly updating them in order to minimize a \emph{loss
function} $\loss: A \to \Real^d\to [0, 1]$.
%

\citet{Hardt} has shown that SGD is
$\left(\frac{2L^2}{n}\sum_{t=0}^{T-1}\alpha_t\right)$\emph{-uniformly
  stable} for suitable loss-functions $\loss$ and step-sizes $\alpha_t$:
for all examples $a\in A$, we have
%
\[
  | \E[\mem]{\sem \sgd_{\mem_S}}{\loss(a,\mem(w))} - \E[\mem]{\sem \sgd_{\mem_{S'}}}{\loss(a,\mem(w))} | \leq \frac{2L^2}{n}\sum_{t=0}^{T-1}\alpha_t,
\]
\noindent
where $\mem_S$ and $\mem_{S'}$ are memories storing
training sets $S$ and $S'$, respectively, that differ in exactly
one example, denoted by $\mem_S \diffone \mem_{S'}$ in the following.

\citet{Aguirre:POPL:21} have proven this statement in their pre-expectation calculus for probabilistic sensitivity.
We re-cast the proof into \ERHLS. As a first step,
a crucial observation is that the absolute distance of two expectations
$|\E{d_1}{f_1} - \E{d_2}{f_2}|$, such as the one expressing algorithmic stability, is bounded from above itself
by the Kantorovich distance $W^\delta_1$ given by the metric $\delta(a_1,a_2) = |f_1(a_1) - f_2(a_2)|$ (see e.g. \cite[Theorem 2.4]{Aguirre:POPL:21}).
By \Cref{rem:krmetric}, a sufficient condition for stability of $\sgd$
is thus given by the \ERHLS\ judgment
\[
  \RHT{a \in A}{\diffone \gd \frac{2L^2}{n}\sum_{t=0}^{T-1}\alpha_t}{\sgd}{\sgd}{\ |{\loss(a, \lft w)} - {\loss(a, \rght w)}|}\,.
\]
To derive this judgment, one can now proceed by reasoning identical to \cite{Aguirre:POPL:21}, using the two-sided rules of \ERHLS.
The invariant computed in \cite{Aguirre:POPL:21} serves essentially as an invariant in the application of Rule~\ref{erhls:While}.


Algorithmic stability of SGD was also established using \EPRHL~\cite{BartheEGHS18}. In comparison to \EPRHL's judgments, those of \ERHL are only meant to reason about expected values, instead of reasoning about sensitivities \emph{and} relational properties. This renders \ERHL's proof system closer to that of \PRHL and thus simpler than \EPRHL's one. As a consequence, \ERHL's proof of SGD's algorithmic stability is simpler than the proof of the same property in \EPRHL.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

